Mutation-based Fault Localization of Deep Neural Networks

Deep neural networks (DNNs) are susceptible to bugs, just like other types of software systems. A significant uptick in using DNN, and its applications in wide-ranging areas, including safety-critical systems, warrant extensive research on software engineering tools for improving the reliability of DNN-based systems. One such tool that has gained significant attention in the recent years is DNN fault localization. This paper revisits mutation-based fault localization in the context of DNN models and proposes a novel technique, named deepmufl, applicable to a wide range of DNN models. We have implemented deepmufl and have evaluated its effectiveness using 109 bugs obtained from StackOverflow. Our results show that deepmufl detects 53/109 of the bugs by ranking the buggy layer in top-1 position, outperforming state-of-the-art static and dynamic DNN fault localization systems that are also designed to target the class of bugs supported by deepmufl. Moreover, we observed that we can halve the fault localization time for a pre-trained model using mutation selection, yet losing only 7.55% of the bugs localized in top-1 position.

==> rebuttal/icse-2023.tex <==
We thank Reviewers for their feedback.
We'll address minor issues in the revision.
Here we clarify doubts and answer questions.

# Review-A:
#### Review-A-C1: "_Results for more bugs[...]_"

Our bug dataset contains representatives of the bug types, e.g., we have _wrong activation function_ bugs at various layers of different types of models for different prediction tasks, and prior works [13,33] have used comparable datasets.
However, we'll add analysis to show representative of our dataset, and add additional bugs if some types aren't well represented.

#### Review-A-Q1: "_Reduce the amount of time required by developers?_"

We can compare the techniques based on $Score$ metric of [*] and calculate the fraction of the program that the developer does _not_ need to examine using each FL technique, i.e., saved time.
We'll supplement the discussion of Section-V.C with the average $Score$ values for each technique: deepmufl(0.768), DeepLocalize(0.139), DeepDiagnosis(0.49), Neuralint(0.279), UMLAUT(0.175), DeepFD(0.21).
deempful has the highest average $Score$ value, indicating bigger expected saving in developer time.

[*] M. Renieris and S. Reiss, "Fault localization with nearest neighbor queries," ICSE'03.

# Review-B:

#### Review-B-C1: "_Adapting MBFL to DL systems must be via meaningful mutators_"
#### Review-B-C2: "_Mutators without any evaluation_"
#### Review-B-C3: "_DeepCrime's mutators emulate real faults_"

We do acknowledge that mutators emulating real faults, better yet traceable mutators, would help generating more informative reports that would also give hints on how to fix the program.
However, unlike mutation analysis, MBFL doesn't depend on _competent programmer hypothesis_ [19,37], so here we aren't necessarily looking for meaningful mutators.
The main objective of an MBFL technique is to assign suspiciousness values to the program elements which can, in theory, be done using _any_ kind of mutator, whether it is meaningful or not (Section-II and [18,29,58]).

#### Review-B-C4: "_DeepMutation++ mutator overlap_"
#### Review-B-C5: "_DeepMutation++ was ignored_"

While we focus on closely related work, we'll explain that there's an overlap between mutators in the two works and why we couldn't reuse some of DeepMutation++'s model-level mutators: some of the model-level mutators offered by DeepMutation++ are already subsumed by deepmufl mutators and we couldn't use others, as they involve (random) shuffling and random weight value mutation, which would make deepmufl non-deterministic/random.

#### Review-B-C6: "_Matching mutators applied to a trained model to a fix on source code_"
#### Review-B-C7: "_If mutant is ranked in top-1, how can it be matched to specific fault?_"

Please kindly note that deepmufl, at this stage, is a proof-of-concept research prototype which prints out ranked layer numbers (and information about the mutations for each layer) for user inspection.
However, given the well-understood structure of Keras programs, with the help of simple auto-generated annotations (e.g., for lexical scoping of the code snippet for model declaration), matching layer numbers to actual lines of code is a matter of putting engineering effort that we'll invest in an extension to this work.

#### Review-B-C8: "_Excluded faults not supported by deepmufl[...]this leads to unfair comparison_"

Despite excluding certain bug types, we argue that our dataset is representative of the bug types that are mostly supported by the baseline approaches, and we can have a fair comparison with the related work.
One of the novelties of our work is the _uniform treatment_ of the models, and our evaluation provides an empirical evidence for this claim.
Please also see **Review-C-C1** and **Review-C-Q1**, below.

#### Review-B-C9: "_How is deepmufl affected by randomness if trained models are used?_"
#### Review-B-C10: "_Because of selected mutators?_"

Training process is stochastic/random; each time, we might get a slightly different model based on the local optima to which the training algorithm has converged, and different models will behave differently when mutated.

Mutation selection is yet another source of randomness that we've taken into account.

#### Review-B-C11: "_Competitor tools are prone to randomness_"

For the bugs that came from the original dataset of each tool, in the rare occasion of observing any discrepancy between the published results and our measurements, we favored the better outcome for baseline techniques (we'll clarify this).
Moreover, given the large margin difference between deepmufl and other tools, we don't think tiny fluctuations in the performance of baseline tools would make them outperform deepmufl.

#### Review-B-C12: "_How much of Humbatova's taxonomy is covered by their dataset_"

Please see the answer to **Review-C-Q3**, below, where we mention examples of bug types that aren't supported by deepmufl, hence aren't included in our dataset.

# Review-C:

#### Review-C-C1: "_The bug benchmark seems biased[...]The following statement should be revised[...]_"
#### Review-C-Q1: "_Does deepmufl results not depend on 60% bug types?"

While we'll rephrase the sentence to make it more specific, we'd like to emphasize that the bugs in the majority class are _not_ similar: they're at different layers of different model types (e.g., CNN, RNN, etc.) and are for different prediction tasks (e.g., regression and classification on different datasets).
Thus, despite having lots of bugs of the same type, we can still have an unbiased comparison with the related work.
One of the novelties of our work is the _uniform treatment_ of models, and our evaluation provides an empirical evidence for this claim: pattern-based DeepDiagnosis, successfully localizes some of the bugs in the majority class yet it fails to generalize, while deepmufl localizes 2+X bugs because it approaches FL problem from a fundamentally different aspect giving it more flexibility.

#### Review-C-C2: "_bug types in replication package_"

We'll add bug types.

#### Review-C-C3: "_Deeper impact of randomness on complex models_"

This limitation can be studied using seeded bugs (currently, we don't have access to more complex real bugs supported by deepmufl) in an extension to this work.

#### Review-C-C4: "_In Section-V.D when they describe why some bugs are not detected[...]Yet it contradicts the point made in Section-VI.B[...]_"

Our first sentence is a bit ambiguous and also misses the possibility of errors being masked by the mutations.
We'll rephrase the sentence.
Here's a clarification: the fact that we didn't observe any difference in the results between different rounds, doesn't mean that randomness in training couldn't have any negative impact on the effectiveness of the approach.
Besides randomness, the mutations in other layers might mask the error in the model and create noise/imprecision in MBFL (as in traditional MBFL).

#### Review-C-Q2: "_The distribution of bugs found per approach and per type?_"

We already have the distribution: deepmulf(Wrong activation function:18, Sub-optimal layer properties:2, Missing/redundant/wrong layer:2), DeepLocalize(Wrong activation function:2, Sub-optimal layer properties:2), DeepDiagnosis(Wrong activation function:12, Sub-optimal layer properties:1, Missing/redundant/wrong layer:1), Neuralint(Wrong activation function:8), DeepDiagnosis(Wrong activation function:8, Missing/redundant/wrong layer:1), and UMLAUT(Wrong activation function:3, Sub-optimal layer properties:1, Missing/redundant/wrong layer:1).
We'd like to add that some of our models in our dataset contain multiple types of bugs.
We'd also like to clarify that by "ablation study" in Future Work, we meant ablation study for _mutators_, which is to be done on a larger dataset to devise heuristic mutation selection rather than random (The reviewer has mentioned this in **Review-C-Q4**).

#### Review-C-Q3: "_Types of bugs detected in previous approaches that aren't detected by deepmufl?_"

4 bugs detected by previous approaches that aren't detected by deepmufl: 3 of type _wrong activation function, while 1 of type _missing/redundant/wrong layer_.
In general, any bug related to data and training hyper-parameters are out of the reach of deepmufl by definition (Section-VI.A)--currently, deepmufl operates on already trained models from which some error-prone information are stripped off.
Some of these bugs are detectable by the existing approaches, but the fact that they're pattern-based, makes them inflexible and we hypothesize that by using source-level mutators offered by DeepCrime, we could detect those bugs also.

#### Review-C-Q4: "_Impact of mutators' distribution on RQ2? If some removed, does it still yield similar results?[...]_"

Answering this question requires further research that we've saved for a future work.


==> tables/sota-details.tex <==
\begin{table}[t]
    \centering
    \caption{Effectiveness of state-of-the-art tools in detecting bugs from four sub-categories of model bugs}
    \resizebox{0.65\columnwidth}{!}{
    \begin{tabular}{c||r|r|r|r||r}
        \textbf{Tool} & \textbf{SC1} & \textbf{SC2} & \textbf{SC3} & \textbf{SC4} & \textbf{Total}\\\hline\hline
        \neuralint & 16 & 0 & 4 & \cellcolor{GrayTwo}1 & 21 \\\hline
        \dl & 21 & 0 & 4 & \cellcolor{GrayTwo}1 & 26 \\\hline
        \dd & \cellcolor{GrayTwo}24 & 0 & 5 & \cellcolor{GrayTwo}1 & 30 \\\hline
        \umlaut & 19 & 0 & \cellcolor{GrayTwo}6 & 0 & 25
    \end{tabular}
    }
    \label{tab:sotaEffectiveness}
\end{table}
